Multimodal Sparse Coding for Event Detection

Unsupervised feature learning methods have proven effective for classification tasks based on a single modality. We present multimodal sparse coding for learning feature representations shared across multiple modalities. The shared representations are applied to multimedia event detection (MED) and evaluated in comparison to unimodal counterparts, as well as other feature learning methods such as GMM supervectors and sparse RBM. We report the cross-validated classification accuracy and mean average precision of the MED system trained on features learned from our unimodal and multimodal settings for a subset of the TRECVID MED 2014 dataset.

==> bg.tex <==
\section{Sparse Coding Background}
Sparse coding is a general class of unsupervised methods to learn efficient representations of data as a linear combination of basis vectors in a dictionary. Given an input (patch) $\mathbf{x} \in \mathbb{R}^N$ drawn from the raw data and an overcomplete dictionary $\mathbf{D}^{N\times K}$ (\ie, $K > N$), sparse coding searches for a representation (\ie, sparse code) $\mathbf{y} \in \mathbb{R}^K$ in the $\ell_1$-regularized optimization $\min_{\mathbf{\mathbf{y}}} \Arrowvert \mathbf{x} - \mathbf{D} \mathbf{y} \Arrowvert^2_2 + \lambda \Arrowvert \mathbf{y} \Arrowvert_1$, known as LASSO or LARS. Greedy-$\ell_0$ matching pursuit such as OMP is an alternative method for sparse coding in $\min_{\mathbf{\mathbf{y}}} \Arrowvert \mathbf{x} - \mathbf{D} \mathbf{y} \Arrowvert^2_2$ s.t. $\Arrowvert \mathbf{y} \Arrowvert_0 \leq S$.    

Dictionary learning is essential for sparse coding. During unsupervised feature learning, we perform sparse coding on unlabeled training examples by holding $\mathbf{D}$ constant. After sparse coding finishes, dictionary updates follow. They will alternate until convergence. Sparse coding can be thought as a generalization of K-means clustering that hard-assigns each training example to one cluster. Sparse coding can also be thought as less stringent, purely data-driven version of Gaussian mixture models.

\comment{
Instructing a classifier with too many features can lead to an undesirable outcome known as overfit. We should subsample sparse codes to their maximum or average feature values. We use \emph{max pooling} that aggregate $\{\mathbf{y}^{(1)},\dots,\mathbf{y}^{(M)}\}$ and yield a pooled sparse code $\mathbf{z}$. The $k$th element in $\mathbf{z}$ is $z_k = \max(y_{k}^{(1)},\dots,y_{k}^{(M)})$ where $y_{k}^{(i)}$ is the $k$th element from $\mathbf{y}^{(i)}$. Essentially, max pooling by $M$ does $\mathbb{R}^{M\times K} \rightarrow \mathbb{R}^K$.
}
